ProNav: Proprioceptive Traversability Estimation for Legged Robot Navigation in Outdoor Environments

We propose a novel method, ProNav, which uses proprioceptive signals for traversability estimation in challenging outdoor terrains for autonomous legged robot navigation. Our approach uses sensor data from a legged robot's joint encoders, force, and current sensors to measure the joint positions, forces, and current consumption respectively to accurately assess a terrain's stability, resistance to the robot's motion, risk of entrapment, and crash. Based on these factors, we compute the appropriate robot gait to maximize stability, which leads to reduced energy consumption. Our approach can also be used to predict imminent crashes in challenging terrains and execute behaviors to preemptively avoid them. We integrate ProNav with an exteroceptive-based method to navigate real-world environments with dense vegetation, high granularity, negative obstacles, etc. Our method shows an improvement up to 40% in terms of success rate and up to 15.1% reduction in terms of energy consumption compared to exteroceptive-based methods.

==> 5_Crash.tex <==
% TODO

%%%%%%%%%%%%%% Should be a new section %%%%%%%%%%%%%%%%%%%%%
\section{ProNav: Crash Handling}
In this section, we analyze the primary causes of locomotion crashes in legged robots. Our analysis reveals two predominant factors that lead to such scenarios: 1. extreme instability in robot movement due to leg \textit{slippage, sinkage, or tripping} incidents, 2. \textit{entrapment} of one or more of the robot legs in vegetation or complex terrains posing an obstruction to continued locomotion. These causes are explored in detail in the subsequent sections.

\subsection{Instability-Induced Crashes}
Further analysis of the PCA graph distributions demonstrated noticeable shifts during the moments immediately before and after crash instances. This trend, visible in Figure \ref{fig:pca_crash}, highlights the direct correlation between these shifts and the occurrence of instability-induced crashes.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.6\columnwidth]{images/PCA_crash4.png}
\caption{\small{Demonstration of two principal component analysis (PCA) components showing significant shifts immediately before and after crash scenarios.}}
\label{fig:pca_crash}
\vspace{-1pt}
\end{figure}

This observation further validates the capability of our chosen proprioceptive parameters (hip actuator position, knee actuator force, and battery current) in identifying varying terrain types and predicting instability induced crashes.

\subsection{Entrapment-Induced Crashes}
Similarly, to understand the causative factors of entrapment-induced crashes, we undertook comprehensive trials where the robot was challenged with entrapment scenarios, specifically within dense vegetation. Unlike previous cases, these experiments necessitated individual analysis of each leg's data. 
Through rigorous analysis, we found that the hip actuator's parameters (position and effort) in the y-axis direction significantly influenced the leg's propensity to become entrapped. Furthermore, the robot's odometry, particularly its linear and angular velocities, played a crucial role in these evaluations.
Our findings suggest that an anomaly between the robot's attempted movements (as indicated by the hip actuator's metrics) and its actual motion (as denoted by the odometry) serves as a robust indicator of possible leg entrapment. Consequently, these parameters can be used to predict entrapment-induced crashes.


%%%%%%%%%%%% Move to section 4 %%%%%%%%%%%%%%%%%%%%%

% \section{Proprioception-based Navigation}
% In this section we discuss our navigation system design in details. We also outline the algorithm for our proposed pseudo haptic navigation. 

% \subsection{\red{Energy-Efficient} Navigation}
% Our navigation system relies on a perception model that incorporates pseudo-haptic sensing to evaluate terrain stability and predict potential crashes. The architecture of the model is divided into two primary modules: \textit{Terrain Assessment} and \textit{Crash Prediction \& Entrapment Detection}. Hence, we formulate our objective as:

% \begin{equation}
% f_{\text{obj}}(t) = \lambda * h^*(.) +  \epsilon * m^*(.)
% \end{equation}

% In this equation:
% $h^*(.)$ represents a function to minimize energy consumption, utilizing stability estimation.

% $m^*(.)$ represents a function to mitigate the risk of potential crashes.

% $\lambda$ and $\epsilon$ are binary scalars. $\lambda$ corresponds to the weight for optimizing energy consumption and $\epsilon$ corresponds to the weight for crash risk mitigation.

% The values of $\lambda$ and $\epsilon$ are determined based on the assessed crash risk. Specifically, if a potential crash is detected, we assign $\epsilon$ = 1 and $\lambda$ = 0. This gives crash prevention priority over energy consumption.

% The following sections provide a detailed discussion on these two main components of our navigation system.

% \subsection{Terrain Assessment}
% We adopt VERN \cite{sathyamoorthy2023vern} to compute the optimal $v^*$ and $w^*$ and determine the most energy-efficient locomotion gait utilizing the following equation.

% \begin{equation}
% \text{{gait}}^* = \arg\min_k h(\text{{gait}}_k, \mathcal{S}(t), v^*, w^*)
% \end{equation}
% where $\text{{gait}}_k$ = [crawl (0), walk (1), ample(2)].

% This gait is chosen based on our comprehensive analysis of various gaits' performances across different terrains, a discussion of which can be found in \red{Appendix A.}


% %Concurrently, the terrain type is categorized as stable/smooth terrain or unstable terrain.
% %sand, rocks, asphalt, concrete, dry grass, or bushes, represented by $t$. 

% If navigation becomes excessively difficult, as denoted by low stability coefficients, the trajectory is adjusted or intermediary waypoints are established in different terrains, guided by a weak segmentation model. 

\subsection{Entrapment Recovery}

The second part predicts crashes and assesses the likelihood of each leg becoming entrapped in dense vegetation. The output comprises four percentages, $e_{1}$, $e_{2}$, $e_{3}$, and $e_{4}$, each corresponding to the front-right, front-left, rear-right, and rear-left legs respectively. To this end, we incorporate a subset of $x_t$, denoted as $z_t$ ($z_t \subseteq x_t$), into the prediction model, and utilize odometry signals represented by $o_t$. These signals help in the determination of the optimal navigation mode (normal operation and recovery).

\begin{equation}
\text{{mode}}^* = \arg\min_k m(\text{{mode}}_k, \mathcal{S}(t), z_t, o_t)
\end{equation}

The robot is switched to recovery mode if the crash percentage surpasses a predefined threshold, $e_{\text{thresh}}$. In the event of entrapment, the robot moves in the reverse right or left (based on the side of the entrapped leg) direction to free that leg. If entanglement events reoccur in the same region, the robot changes its path or sets up a new waypoint according to the weak segmentation model, reducing the potential for crashes and enhancing operational safety.

\subsection{Algorithm Design}

The designed algorithm for our navigation system is described in algorithm 1.

\begin{algorithm}
\caption{ProNav Navigation}
\begin{algorithmic}[1]
\For {each time $t$}
    \State Compute $f(\sigma_{PC1}, \sigma_{PC2}) \gets \text{TerrainAssessment}(.)$
    \State Compute $v^*, w^* \gets \text{VERN}(.)$
    \If {$\mathcal{f}(.) > f_{\mathrm{thresh}}$} 
        \State Compute $g^* = \underset{g \in \{\text{Amble, Crawl}\}}{\operatorname{argmin}} h(g)$
    \EndIf
    \For {each leg $i$}
        \State Compute $e_{i} \gets \text{Entrapment Detection}(i)$
        \If {$e_{i} > e_{\mathrm{thresh}}$}
            \State Initiate recovery mode
        \EndIf
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


This approach enables the robot to safely navigate varied terrains while considerably minimizing the risk of crashes due to leg entrapments.


==> 8_Acknowledgement.tex <==
\section{Acknowledgement}
